E3D: Event-Based 3D Shape Reconstruction

3D shape reconstruction is a primary component of augmented/virtual reality. Despite being highly advanced, existing solutions based on RGB, RGB-D and Lidar sensors are power and data intensive, which introduces challenges for deployment in edge devices. We approach 3D reconstruction with an event camera, a sensor with significantly lower power, latency and data expense while enabling high dynamic range. While previous event-based 3D reconstruction methods are primarily based on stereo vision, we cast the problem as multi-view shape from silhouette using a monocular event camera. The output from a moving event camera is a sparse point set of space-time gradients, largely sketching scene/object edges and contours. We first introduce an event-to-silhouette (E2S) neural network module to transform a stack of event frames to the corresponding silhouettes, with additional neural branches for camera pose regression. Second, we introduce E3D, which employs a 3D differentiable renderer (PyTorch3D) to enforce cross-view 3D mesh consistency and fine-tune the E2S and pose network. Lastly, we introduce a 3D-to-events simulation pipeline and apply it to publicly available object datasets and generate synthetic event/silhouette training pairs for supervised learning.

==> E3D/Thesis/abstract.tex <==
\thispagestyle{plain}
\begin{center}
    \Large
    E3D: Event-Based 3D Shape Reconstruction
    
    \vspace{0.4cm}
    \large
    Alexis Baudron
    
    \vspace{1cm}
    \Large
    Abstract
\end{center}
 3D shape reconstruction is a primary component of augmented/virtual reality. Despite being highly advanced, existing solutions based on RGB, RGB-D and Lidar sensors are power and data intensive, which introduces challenges for deployment in edge devices. We approach 3D reconstruction with an event camera, a sensor with significantly lower power, latency and data expense while enabling high dynamic range. While previous event-based 3D reconstruction methods are primarily based on stereo vision, we cast the problem as multi-view shape from silhouette using a monocular event camera. The output from a moving event camera is a sparse point set of space-time gradients, largely sketching scene/object edges and contours. In this thesis, we first introduce an event-to-silhouette (E2S) neural network module to transform a stack of event frames to the corresponding silhouettes, with additional neural branches for camera pose regression. Second, we introduce E3D, which employs a 3D differentiable renderer (PyTorch3D) to enforce cross-view 3D mesh consistency and fine-tune the E2S and pose network. Lastly, we introduce a 3D-to-events simulation pipeline and apply it to publicly available object datasets and generate synthetic event/silhouette training pairs for supervised learning. Additionally, we evaluate our pipeline on challenging real event data collected with a CeleX camera. 

==> E3D/Thesis/title.tex <==
%%%%%%%%% TITLE
\begin{titlepage}
    \begin{center}
        NORTHWESTERN UNIVERSITY
        
        \vspace{1.5cm}
        E3D: Event-Based 3D Shape Reconstruction

        \vspace{1.5cm}
        A PROJECT
        
        \vspace{.5cm}
        SUBMITTED TO THE GRADUATE SCHOOL IN PARTIAL FULFILLMENT OF THE REQUIREMENTS
        
        \vspace{1cm}
        for the degree
        
        \vspace{1cm}
        MASTERS OF SCIENCE
        
        \vspace{1cm}
        Field of Computer Science
            
        \vspace{1cm}
        By \\
        Alexis Baudron
        
        \vspace{1cm}
        EVANSTON, ILLINOIS
        
        \vspace{1cm}
        December 2020
            
    \end{center}
\end{titlepage}


==> E3D/WhitePaper.tex <==
\begin{abstract}
    In this paper we propose a method for recovering an object's 3D shape from an event camera. An event camera is a differential sensor that responds to local changes in brightness, it has microsecond temporal resolution, high dynamic range and does not suffer from under or overexposure. Accurately recovering shape from scenes has been a long-standing problem in Computer Vision. We focus on evaluating monocular image-based approaches to constrain our study to sensors that do not immediately provide depth information. In recent years, learning approaches have enabled single-view and sparse multi-image shape reconstruction. Other approaches make the rendering process differentiable to train the reconstruction model from RGB images. Unfortunately, these approaches are restricted to the limitations of the camera sensor, failing in extreme lighting conditions, suffering from motion blur and high memory and power consumption. We propose leveraging the advantages of the event camera to bring robust, high-speed shape recovery from a 3D scene. In this paper we will discuss our proposed approaches, anticipated milestones and bottlenecks.
\end{abstract}

\begin{abstract}
    In this paper we propose a method for recovering an object's 3D shape from an event camera. \alexis{An event camera is a differential sensor that responds to local changes in brightness, it has microsecond temporal resolution, high dynamic range and does not suffer from under or overexposure}. Accurately recovering shape from scenes has been a long-standing problem in Computer Vision. We focus on evaluating monocular image-based approaches to constrain our study to sensors that do not immediately provide depth information. In recent years, learning approaches have enabled single-view and sparse multi-image shape reconstruction. Other approaches make the rendering process differentiable to train the reconstruction model from RGB images. Unfortunately, these approaches are restricted to the limitations of the camera sensor, failing in extreme lighting conditions, suffering from motion blur and high memory and power consumption. We propose leveraging the advantages of the event camera to bring robust, high-speed shape recovery from a 3D scene. In this paper we will discuss our proposed approaches, anticipated milestones and bottlenecks. \winston{ordering: 3d problem -- issues -- solutions}\winston{title runner-up: E3D: Event-based 3D Object Shape Reconstruction}
\end{abstract}

\begin{abstract}
    3D shape estimation and tracking is a primary component of mixed reality applications. Despite recent advances in neural hardware architectures and sensor design that have enabled moving these algorithms to wearable devices, mixed reality glasses or phones are still resource constrained when handling the sensors and algorithms powering these applications. RGB, RGB-D and Lidar are commonly used sensors for tackling AR/VR, but they are both power and data intensive (1W/32MB.$s^{-1}$ & >2W/??? & 4W/100MB.$s^{-1}$), introducing significant engineering challenges when designing these devices. Core engineering and algorithm innovation such as new shape parameterizations have been at the forefront of solving this problem. We propose using an event camera, a bio-inspired neuromorphic sensor that responds to local changes in brightness with very low power consumption (1mW) and low data bandwidth (1MB.$s^{-1}$), to recover 3D object shape and camera pose. Our category-specific approach leverages multiple-views to build a triangular mesh of the object by learning mask priors from the event stream. We use a gradient-based mesh editing approach to optimize our recovered mesh using the inferred silhouettes and camera pose during supervision. We train our pipeline in simulation and test the robustness of our approach on unseen views and environments with both synthetic and real data.  
\end{abstract}


\section{Event Camera - How it works}
Event cameras respond to brightness changes in the scene, with each pixel on the event camera responding asynchronously and independently. This processing approach is inspired by human vision by modeling visual pathways in the human brain. \\
In a noise free scenario, a single event $e_k$, triggered at pixel $\bold{X}_k = (x_k, y_k)$ contains the following information.
\begin{equation}
    e_k = [t_k, \bold{X}_k, p_k]
\end{equation} 
where the timestamp $t_k$ is in $\mu s$ and polarity $p_k \in \{ -1, 1\}$ is the sign of the brightness change.
The event is triggered if the brightness change since the last event: 
\begin{equation}
    \Delta L (\bold{X}_k, t_k) = L(\bold{X}_k, t_k) - L(\bold{X}_k, t_k - \Delta t_k) 
\end{equation} 
is above a temporal contrast threshold $\pm C$:
\begin{equation}
     \Delta L (\bold{X}_k, t_k) = p_k C
\end{equation}
where C $>$ 0 and is usually determined by an on-chip bias generator. As such an event can be triggered according to different thresholds. With low values of C, the event sensor picks up small changes in brightness which generates a lot of noise. The event sensor measures a temporal derivative of brightness, for a small $\Delta t_k$ we can use Taylor's expansion to approximate: $\Delta L (\bold{X}_k, t_k) \approx \frac{\delta L}{\delta t}(\bold{X}_k, t_k)$. As such the event camera only sees what "changes" in the scene (fig. \ref{fig:output}). If an object is moving through a room, the only brightness change that occurs is between the object and the background, at the boundary of the object (fig. \ref{fig:motioncomparison} \& \ref{fig:nomotioncomparison}). 
For a detailed survey on event cameras we refer to ~\cite{gallego2019eventbased}.
\winston{I don't see this paragraph relevant. Afterall, you don't pick up this math later.}

\textbf{High-Speed Motion Capture with an event camera}
EventCap ~\cite{xu2019eventcap} proposes a method to do high speed human pose tracking, their approach consists of generating intensity frames from the event stream, they recover the 2D and 3D joint positions using OpenPose ~\cite{cao2018openpose}, a realtime pose estimation algorithm. They use the event-based asynchronous feature tracker in ~\cite{Gehrig_2018} to track features relevant to joint positions in the frame as the body moves. Although this work is a good example of leveraging the temporal resolution of the event camera, the authors reconstruct intensity frames from events to recover the human pose. Events are binned into discretized frames to create an intensity, losing temporal information in the process. \newline

\subsection{Differentiable Rendering}
Rendering is the process of creating a photo-realistic image from a known 3D shape. Inverse rendering is the process of recovering 3D shape from a single or multiple reference images. \\

\textbf{Mesh: }
Attempts at recovering a mesh were first introduced by OpenDR ~\cite{opendr_2014} which uses Automatic Differentiation on appearance and geometry to recover a triangular mesh of the object. Neural 3D Resh Renderer ~\cite{kato2017neural}, proposes a gradient descent algorithm that learns to deform a template mesh via 2D silhouette and smoothness loss. Soft Rasterizer ~\cite{liu2019soft}, extends ~\cite{kato2017neural} by proposing a fully differentiable soft rasterizer suitable for neural networks. With recent advances in convolution networks, there have been very successful works taking into consideration rendering approaches in deep learning frameworks. Such approaches include a differential rendering layer in their architecture such as DIB-R ~\cite{chen2019learning}.

\textbf{Neural Mesh: }
The image to mesh approach described in ~\cite{henderson2020leveraging} contributes two networks, the first a generative model that learns to generate 3D textured shapes, the second a network that includes a differentiable renderer layer that provides a reconstruction loss for training this model. To adapt this method to events we would take the encoder, composed of small CNN to extract features and only use the shape decoder composed of an ELU network. See Fig \ref{img2mesh}.  
\begin{figure}[t]
  \centering
  \includegraphics[scale=.3]{E3D - White Paper/img2mesh.png}
  \caption{Architecture Diagram of Henderson, et al ~\cite{henderson2020leveraging}}
  \label{img2mesh}
\end{figure}

\textbf{Voxels: }
The mesh-based methods require an initial template mesh and then learn to deform it progressively by minimizing the reconstruction loss. Some approaches have shown that voxels are also a good candidate in differentiable rendering pipelines. Rematas et al ~\cite{rematas2019neural} build on the work of RenderNet ~\cite{nguyenphuoc2018rendernet} to create a high quality Neural Voxel Renderer that uses a differentiable layer. Because of their grid like structure voxels are easily processed by deep learning architectures. A recent approach described in ~\cite{Park_2020_CVPR} creates a latent 3D voxel grid from a set of $N$ measurements as a means of recovering camera pose parameters. They start by creating a set of feature volumes (voxels) from each view and fuse them together using an RNN unit. Next, they render the voxels in an approach similar to RenderNet ~\cite{nguyenphuoc2018rendernet} using sets of 2D and 3D U-Nets ~\cite{ronneberger2015unet}. Fig. \ref{latfusion} is a diagram of the architecture.
\begin{figure}[h]
  \centering
  \includegraphics[scale=.3]{E3D - White Paper/latent_vox2020.png}
  \caption{Latent Fusion ~\cite{Park_2020_CVPR} Architecture Diagram}
  \label{latfusion}
\end{figure}
Although voxels can be easily approximated from a set of measurements without the need for an initial mesh, they do not extend well to large objects being limited by their resolution.

\textbf{Implicit Representations: }
Implicit neural representations have gained popularity for learning-based neural rendering. Occupancy networks are introduced in ~\cite{mescheder2018occupancy} as binary networks that encode the probability of a point at the boundary of the objects. This representation is capable of encoding details that are lost in voxel-based 3D representations. More recently, Niemeyer et al ~\cite{niemeyer2019differentiable}, use a Differential Volumetric rendering approach to learn the occupancy network of an object from single views. They define a photometric reconstruction loss from which they can learn the occupancy network from a groundtruth 2D image. Their approach is fully differentiable and their training approach consists of first sampling points on the image. For the case of events we could use points on the boundary of the object instead. Other implicit representations such as Scene Representation Networks in ~\cite{scene_network2019} are differentiable and could be a potential research path into recovering an implicit 3D representation from events.
